Safe Serializable Secure Scheduling: Transactions and the Trade-off Between Security and Consistency

Modern applications often operate on data in multiple administrative domains. In this federated setting, participants may not fully trust each other. These distributed applications use transactions as a core mechanism for ensuring reliability and consistency with persistent data. However, the coordination mechanisms needed for transactions can both leak confidential information and allow unauthorized influence. By implementing a simple attack, we show these side channels can be exploited. However, our focus is on preventing such attacks. We explore secure scheduling of atomic, serializable transactions in a federated setting. While we prove that no protocol can guarantee security and liveness in all settings, we establish conditions for sets of transactions that can safely complete under secure scheduling. Based on these conditions, we introduce staged commit, a secure scheduling protocol for federated transactions. This protocol avoids insecure information channels by dividing transactions into distinct stages. We implement a compiler that statically checks code to ensure it meets our conditions, and a system that schedules these transactions using the staged commit protocol. Experiments on this implementation demonstrate that realistic federated transactions can be scheduled securely, atomically, and efficiently.

==> blindtr.tex <==
\def\paperversion{blindtr}
\def\anonymoussubmission{1} % remove or change to 0 to make submission non-anonymous
\input{paperversions}
\input{header}
\begin{document}
\input{body}
\end{document}


==> make/commondefs <==
#
# See the manual page for "commondefs" for more information.
#

INCLDIR = $(ROOT)/usr/include
TEXDIR = ../tex-macros

COMMONRULES = $(MAKEDIR)/commonrules

SOURCES = $(CFILES) $(C++FILES) $(YFILES) $(LFILES) $(AFILES)
OBJECTS = $(CFILES:.c=.o) $(C++FILES:.C=.o)
DIRT = *.o core *.aux* *.dvi *.log *.stamp *.i *.bbl *.out *.upa *.upb *.[ib]lg $(LDIRT)
GENERATED = .dependtime Makedepend Makedepend.bak
RM = rm -f
MKDEPFILE = Makedepend
MKDEPEND = makedepend
MKDEPFLAGS = -Y
MKDEPC++FLAGS = $(C++DEFS) $(C++INCS) $(MKDEPFLAGS)
MKDEPCFLAGS = $(CDEFS) $(CINCS) $(MKDEPFLAGS)

.SUFFIXES: .C .ps .i .txt .h
.SUFFIXES: .tex .dvi .ind .idx .bbl .aux .glo .aux .stamp .pdf .eps

GNUBIN = /usr/local

ATTC++ = CC
DECC++ = cxx
GNUC++ = g++

CC = cc
C++ = $(GNUC++)
YACC = bison
DVIPS = dvips

C++F = $(C++) $(C++FLAGS)
CCF = $(CC) $(CFLAGS)

C++FLAGS = $(C++OPTS) $(C++DEFS) $(C++INCS)

C++INCS = $(GC++INCS) $(LC++INCS)
C++OPTS = $(GC++OPTS) $(LC++OPTS)
C++DEFS = $(GC++DEFS) $(LC++DEFS)

GC++OPTS = $(OPTIMIZER)

CFLAGS = $(COPTS) $(CDEFS) $(CINCS)
COPTS = $(GCOPTS) $(LCOPTS)
CDEFS = $(GCDEFS) $(LCDEFS)
CINCS = $(GCINCS) $(LCINCS)

GCOPTS = $(OPTIMIZER)

M3F = $(M3) $(M3FLAGS)
M3 = m3
M3PP = m3pp

LDFLAGS = $(LLDFLAGS) $(GLDFLAGS)
LLDFLAGS = $(LLDLIBS) $(LLDOPTS) 

SEP=:
#SEP=\;         # for MikTeX+Cygwin # Deprecated: define this in $(MAKEDIR)/localdefs
TEXINPUTS = .$(SEP)$(TEXDIR)$(SEP)
LATEX = TEXINPUTS='$(TEXINPUTS)' latex --output-directory='$(BUILD)'
PDFLATEX = TEXINPUTS='$(TEXINPUTS)' pdflatex --output-directory='$(BUILD)'
BIBTEX = bibtex

# Directory for TeX's generated files.
BUILD = .
# BUILDD should be equivalent to $(BUILD)/
BUILDD =
VPATH = $(BUILD)

-include localdefs


==> make/commonrules <==
# Some basic recursive rules for building, installing, and cleaning up
# a source tree
#
subdirs:
	@sub="$(SUBDIRS)"; \
	for i in $$sub; do if test -n "$$i"; then \
	      (cd $$i; make); \
	fi; done;

clean:  localclean
	@sub="$(SUBDIRS)"; \
	for i in $$sub; do if test -n "$$i"; then \
	      (cd $$i; make $@); \
	fi; done;

localclean:
	$(RM) $(DIRT)

clobber: localclean
	@sub="$(SUBDIRS)";						      \
	for i in $$sub; do if test -n "$$i"; then			      \
	      (cd $$i; make $@);					      \
	fi; done;
	$(RM) $(TARGETS) $(GENERATED)

install: default localinstall
	@sub="$(SUBDIRS)";						      \
	for i in $$sub; do if test -n "$$i"; then			      \
	      (cd $$i; make $@);					      \
	fi; done;

incdepend: .dependtime
depend: .dependtime

.dependtime: $(SOURCES)
	touch temp
	$(MKDEPEND) $(MKDEPC++FLAGS) -f temp $(C++FILES)
	touch $(MKDEPFILE)
	$(MKDEPEND) $(MKDEPCFLAGS) -f $(MKDEPFILE) $(CFILES)
	cat temp >> $(MKDEPFILE)
	$(RM) temp
	touch $@

# Rules for TeX files
#
# The line that runs LATEX needs to run inside a subshell to turn off
# "make"'s status checking. It blows away .aux because the .aux file
# created is bad and also breaks bibtex. It touches .stamp to force a
# rebuild.
.tex.dvi:
	@if test -r "$*.aux";						      \
	   then cp "$(BUILDD)$*.aux" "$(BUILDD)$*.auxprev";		      \
	   else echo > "$(BUILDD)$*.auxprev";				      \
	fi
	@echo "$(LATEX) $<"
	@sh -c "$(LATEX) $< || ($(RM) $*.aux; sleep 1; touch \"$(BUILDD)$*.stamp\"; exit 1)"
	@-cmp -s "$(BUILDD)$*.aux" "$(BUILDD)$*.auxprev";		      \
	if test $$? = 1;						      \
	then								      \
	    sleep 1;							      \
	    echo "==> Rebuilding $@";					      \
	    touch "$(BUILDD)$*.stamp";					      \
	    $(MAKE) $@;							      \
	else								      \
	    echo "==> No need to rebuild $@";				      \
	fi
	@$(RM) "$(BUILDD)$*.auxprev"

.tex.pdf:
	@if test -r "$(BUILDD)$*.aux";					      \
	   then cp "$(BUILDD)$*.aux" "$(BUILDD)$*.auxprev";		      \
	   else echo > "$(BUILDD)$*.auxprev";				      \
	fi
	@echo "$(PDFLATEX) $<"
	@sh -c "$(PDFLATEX) $< || ($(RM) $*.aux; sleep 1; touch \"$(BUILDD)$*.stamp\"; exit 1)"
	@-cmp -s "$(BUILDD)$*.aux" "$(BUILDD)$*.auxprev";		      \
	if test $$? = 1;						      \
	then								      \
	    sleep 1;							      \
	    echo "==> Rebuilding $@";					      \
	    touch "$(BUILDD)$*.stamp";					      \
	    $(MAKE) $@;							      \
	else								      \
	    echo "==> No need to rebuild $@";				      \
	fi
	@$(RM) "$(BUILDD)$*.auxprev"

# must add dependencies like
#    foo.ind: foo.stamp
#    foo.dvi: foo.ind
# to use this rule properly.
.tex.ind:
	@if [ -f $*.idx ]; then						      \
	   echo makeindex $*.idx;					      \
	   makeindex $*.idx;						      \
	else								      \
	   echo touch $@;						      \
	   touch $@;							      \
        fi

# must add dependencies like
#    foo.bbl: foo.bib
#    foo.dvi: foo.bbl
# to use this rule properly.
.tex.bbl:
	@if [ -r $*.aux ]; then echo $(BIBTEX) $*; sh -c "$(BIBTEX) $* || echo"; else echo; fi

.tex.stamp: # backward compatibility
	touch $@

.dvi.ps:
	$(DVIPS) $(DVIPSOPTS) $< -o $@
.eps.pdf:
	epstopdf $(EPSTOPDFOPTS) $<

#
# Rules for C++ and .i files
#

.C.i:
	$(C++F) -E $< > $@

.c.i:
	$(CCF) -E $< > $@

.C.o:
	$(C++F) -c $<

# include $(M3SU)    # old Modula-3 rules

# Paper versions
markup:
	@DOC=markup MAKEFLAGS=e $(MAKE)
draft:
	@DOC=draft MAKEFLAGS=e $(MAKE)
tr:
	@DOC=tr MAKEFLAGS=e $(MAKE)
trdraft:
	@DOC=trdraft MAKEFLAGS=e $(MAKE)
local:
	@DOC=local MAKEFLAGS=e $(MAKE)
submission:
	@DOC=submission MAKEFLAGS=e $(MAKE)
final:
	@DOC=final MAKEFLAGS=e $(MAKE)
finaldraft:
	@DOC=finaldraft MAKEFLAGS=e $(MAKE)
blindtr:
	@DOC=blindtr MAKEFLAGS=e $(MAKE)
web:
	@DOC=web MAKEFLAGS=e $(MAKE)


==> markup.tex <==
\def\paperversion{markup}
\def\anonymoussubmission{1} % remove or change to 0 to make submission non-anonymous
\input{paperversions}
\input{header}
\begin{document}
\input{body}
\end{document}


==> paper.tex <==
\def\paperversion{DOC}
\def\anonymoussubmission{1} % remove or change to 0 to make submission non-anonymous
\input{paperversions}
\input{header}
\begin{document}
\input{body}
\end{document}


==> report.tex <==
\def\paperversion{report}
\def\anonymoussubmission{1} % remove or change to 0 to make submission non-anonymous
\input{paperversions}
\input{header}
\begin{document}
\input{body}
\end{document}

